Non-Detections of Helium in the Young Sub-Jovian Planets K2-100b, HD 63433b, & V1298 Tau c

We search for excess in-transit absorption of neutral helium at 1.083 $\mu$m in the atmospheres of the young (<800 Myr) sub-Jovian (0.2-0.5 $\rm R_{J}$) planets HD 63433b, K2-100b, and V1298 Tau c using high-resolution (R~25,000) transit observations taken with Keck II/NIRSPEC. Our observations do not show evidence of helium absorption for any of the planets in our sample. We calculate 3$\sigma$ upper limits on the planets' excess helium absorption of <0.47% for HD 63433b, <0.56% for K2-100b, and <1.13% for V1298 Tau c. In terms of equivalent width, we constrain these to <2.52, <4.44, and <8.49 mA for HD 63433b, K2-100b, and V1298 Tau c, respectively. We fit our transmission spectra with one-dimensional Parker wind models to determine upper limits on the planets' mass-loss rates of <7.9$\times10^{10}$, <1.25$\times10^{11}$, and <$7.9\times10^{11}$g s$^{-1}$. Our non-detections align with expectations from one-dimensional hydrodynamic escape models, magnetic fields, and stellar wind confinement. The upper limits we measure for these planets are consistent with predicted trends in system age and He equivalent width from 1D hydrodynamic models.

==> tab_flux_params.tex <==
\begin{table*}
\caption{Integrated fluxes received by each planet over the X-ray [0.517-12.4 nm], hard-EUV [10-36 nm], soft-EUV [36-92 nm] and mid-UV [91.2-320 nm] bands in the model of \citet{Allan23}. }
  \centering
  \begin{tabular}{ccccccccccccccccc}
  		% \hline 
    % \hline 
 Name             & $ F_{\rm X-ray}$   &  $   F_{\rm hEUV} $   & $ F_{\rm sEUV} $      & $ F_{\rm mid-UV} $        \\
           & (erg/s/cm$^2$)     &  (erg/s/cm$^2$)    & (erg/s/cm$^2$)      & (erg/s/cm$^2$)        \\
           \hline
HD 63433b  & 5.39$\times$10$^{3}$  &  4.64$\times$10$^{3}$  &  6.75$\times$10$^{3}$  &  5.33$\times$10$^{6}$   \\
V1298\,Tau\,c  &    1.84$\times$10$^{5}$  &  3.75$\times$10$^{4}$  &  1.73$\times$10$^{4}$  &  1.19$\times$10$^{6}$    \\
K2-100b &    1.98$\times$10$^{4}$  &  1.70$\times$10$^{4}$  &  4.60$\times$10$^{4}$  &  3.21$\times$10$^{6}$    \\
% \hline
\end{tabular}
\label{tab_flux_params}
\end{table*}
